Using Large Language Models for (De-)Formalization and Natural Argumentation Exercises for Beginner's Students

We describe two systems currently being developed that use large language models for the automatized correction of (i) exercises in translating back and forth between natural language and the languages of propositional logic and first-order predicate logic and (ii) exercises in writing simple arguments in natural language in non-mathematical scenarios.

==> eptcsdata.tex <==
\providecommand{\firstpage}{28}
\providecommand{\publicationstatus}{J. Narboux, W. Neuper and P. Quaresma (Eds.): Workshop on\\ Theorem proving components for Educational software 2023 (ThEdu'23)\\
EPTCS 400, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.400.3}{10.4204/EPTCS.400.3}}
\pdfoutput=1

